A Refined Estimate of the Ionizing Emissivity from Galaxies at z~3: Spectroscopic Follow-up in the SSA22a Field

We investigate the contribution of star-forming galaxies to the ionizing background at z~3, building on previous work based on narrowband (NB3640) imaging in the SSA22a field. We use new Keck/LRIS spectra of Lyman break galaxies (LBGs) and narrowband-selected Lya emitters (LAEs) to measure redshifts for 16 LBGs and 87 LAEs at z>3.055, such that our NB3640 imaging probes the Lyman-continuum (LyC) region. When we include the existing set of spectroscopically-confirmed LBGs, our total sample with z>3.055 consists of 41 LBGs and 91 LAEs, of which nine LBGs and 20 LAEs are detected in our NB3640 image. With our combined imaging and spectroscopic data sets, we critically investigate the origin of NB3640 emission for detected LBGs and LAEs. We remove from our samples 3 LBGs and 3 LAEs with spectroscopic evidence of contamination of their NB3640 flux by foreground galaxies, and statistically model the effects of additional, unidentified foreground contaminants. The resulting contamination and LyC-detection rates, respectively, are 62 +/-13% and 8 +/-3% for our LBG sample, and 47 +/-10% and 12 +/-2% for our LAE sample. The corresponding ratios of non-ionizing UV to LyC flux-density, corrected for intergalactic medium (IGM) attenuation, are 18.0 +34.8/-7.4 for LBGs, and 3.7 +2.5/-1.1 for LAEs. We use these ratios to estimate the total contribution of star-forming galaxies to the ionizing background and the hydrogen photoionization rate in the IGM, finding values larger than, but consistent with, those measured in the Lya forest. Finally, the measured UV to LyC flux-density ratios imply model-dependent LyC escape fractions of f_{esc}^{LyC} ~ 5-7% for our LBG sample and f_{esc}^{LyC} ~ 10-30% for our fainter LAE sample.

==> tab3.tex <==
\begin{deluxetable}{ccccccccc}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Summary of LAE Data \label{t:3}}
\tablehead{
\colhead{ID} & \colhead{RA} & \colhead{Dec}  & \colhead{$R$} & \colhead{NB3640} & \colhead{$\Delta_R$\tablenotemark{a}} & \colhead{$\Delta_{LyA}$\tablenotemark{a}} & \colhead{$\frac{F_{UV}}{F_{LyC}}_{obs}$\tablenotemark{b}} & \colhead{$z_{em}$\tablenotemark{c}} \\
 & \colhead{(J2000)} & \colhead{(J2000)} & & & & &  &
}
\startdata
001\tablenotemark{d,e} & 22:17:32.40 & 0:11:34.1 & 23.92 & $>27.3$ & \ldots & \ldots & $>22.4$ & 3.075 \\
002\tablenotemark{d,e} & 22:17:38.90 & 0:11:01.8 & 24.28 & $>27.3$ & \ldots & \ldots & $>16.2$ & 3.076 \\
003 & 22:17:24.79 & 0:17:17.4 & 24.42 & 24.74\tablenotemark{f} & 0\secpoint3 & 0\secpoint6 & \ldots & 3.097\\
004\tablenotemark{d,e} & 22:17:28.01 & 0:14:30.0 & 24.34 & $>27.3$ & \ldots & \ldots & $>15.2$ & 3.092 \\
005 & 22:17:35.86 & 0:15:59.4 & 25.65 & $>27.3$ & \ldots & \ldots & $>4.6$ & 3.096 \\
006 & 22:17:24.80 & 0:11:16.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.071 \\
007 & 22:17:27.78 & 0:17:36.9 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.089 \\
008\tablenotemark{d,e} & 22:17:21.11 & 0:15:28.0 & 24.87 & $>27.3$ & \ldots & \ldots & $>9.3$ & 3.076 \\
009\tablenotemark{d} & 22:17:28.29 & 0:12:12.3 & 25.84 & $>27.3$ & \ldots & \ldots & $>3.8$ & 3.071 \\
010 & 22:17:20.38 & 0:18:04.2 & 25.77 & 26.74 & 0\secpoint3 & 0\secpoint3 & $2.4\pm1.1$ & 3.096 \\
011 & 22:17:33.85 & 0:12:14.9 & 26.07 & $>27.3$ & \ldots & \ldots & $>3.1$ & 3.102 \\
012\tablenotemark{d,e} & 22:17:31.69 & 0:16:57.6 & 24.75 & $>27.3$ & \ldots & \ldots & $>10.5$ & 3.094 \\
013 & 22:17:27.18 & 0:16:21.7 & 25.98 & $>27.3$ & \ldots & \ldots & $>3.4$ & 3.095 \\
014 & 22:17:19.25 & 0:14:50.9 & 25.82 & $>27.3$ & \ldots & \ldots & $>3.9$ & 3.067 \\
015 & 22:17:21.84 & 0:12:12.7 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.067 \\
016 & 22:17:35.61 & 0:18:00.2 & 26.24 & 26.91 & 0\secpoint9 & 0\secpoint8 & $1.8\pm0.9$ & 3.091 \\
017 & 22:17:25.40 & 0:17:16.8 & 26.22 & $>27.3$ & \ldots & \ldots & $>2.7$ & 3.105 \\
018 & 22:17:39.01 & 0:17:26.4 & 26.25 & 25.69 & 0\secpoint1 & 1\secpoint0 & $0.6\pm0.2$ & 3.093 \\
019 & 22:17:26.15 & 0:13:20.1 & 25.70 & 26.24\tablenotemark{f} & 0\secpoint4 & 0\secpoint9 & \ldots & 3.101 \\
020 & 22:17:37.33 & 0:16:31.4 & 25.45 & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{g} \\
021 & 22:17:18.77 & 0:15:18.1 & $>27.0$ & 27.17 & 1\secpoint3 & 1\secpoint4 & $<1.8$ & 3.070 \\
022 & 22:17:19.68 & 0:11:49.4 & 26.11 & $>27.3$ & \ldots & \ldots & $>3.0$ & 3.066 \\
023 & 22:17:31.73 & 0:16:06.9 & 24.91 & $>27.3$ & \ldots & \ldots & $>9.1$ & 3.101 \\
024 & 22:17:34.17 & 0:16:09.7 & 26.73 & $>27.3$ & \ldots & \ldots & $>1.7$ & 3.096 \\
025 & 22:17:36.74 & 0:16:28.8 & 25.54 & 25.85\tablenotemark{f} & 0\secpoint3 & 1\secpoint2 & \ldots & 3.091\\
026 & 22:17:18.96 & 0:12:00.8 & 26.59 & $>27.3$ & \ldots & \ldots & $>1.9$ & 3.092 \\
027 & 22:17:24.94 & 0:17:17.3 & 26.25 & $>27.3$ & \ldots & \ldots & $>2.6$ & 3.101 \\
028 & 22:17:31.80 & 0:17:17.9 & 25.50 & 26.71 & 0\secpoint3 & 0\secpoint9 & $3.1\pm1.3$ & 3.088 \\
029\tablenotemark{d} & 22:17:31.49 & 0:12:55.0 & 25.38 & $>27.3$ & \ldots & \ldots & $>5.9$ & 3.107 \\
030 & 22:17:21.75 & 0:11:38.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.096 \\
031 & 22:17:33.63 & 0:17:15.1 & 26.37 & $>27.3$ & \ldots & \ldots & $>2.3$ & 3.092 \\
032 & 22:17:26.61 & 0:13:18.1 & 26.61 & $>27.3$ & \ldots & \ldots & $>1.9$ & 3.101 \\
033 & 22:17:37.50 & 0:14:08.3 & 26.62 & $>27.3$ & \ldots & \ldots & $>1.9$ & 3.076 \\
034 & 22:17:23.41 & 0:16:35.4 & 25.42 & 25.76\tablenotemark{h} & 0\secpoint5 & 0\secpoint0 & $1.4\pm0.4$ & 3.044\\
035 & 22:17:27.03 & 0:13:13.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.093 \\
036 & 22:17:22.25 & 0:11:55.1 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.084 \\
037 & 22:17:20.96 & 0:18:07.3 & 25.61 & $>27.3$ & \ldots & \ldots & $>4.7$ & 3.089 \\
038 & 22:17:34.77 & 0:15:41.3 & 26.17 & 25.82 & 0\secpoint1 & 0\secpoint7 & $0.7\pm0.3$ & 3.099 \\
039 & 22:17:24.08 & 0:11:31.7 & 26.48 & 26.77 & 0\secpoint4 & 0\secpoint8 & $1.3\pm0.7$ & 3.095 \\
040 & 22:17:31.93 & 0:13:08.5 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.105 \\
041 & 22:17:24.54 & 0:15:06.7 & 25.97 & 25.94 & 0\secpoint4 & 0\secpoint5 & $1.0\pm0.4$ & 3.066 \\
042 & 22:17:21.50 & 0:17:04.7 & 25.50 & $>27.3$ & \ldots & \ldots & $>5.2$ & 3.072 \\
043 & 22:17:21.65 & 0:12:23.4 & 26.24 & $>27.3$ & \ldots & \ldots & $>2.7$ & 3.071 \\
044 & 22:17:36.41 & 0:12:51.0 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.059 \\
045 & 22:17:35.97 & 0:16:30.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.094 \\
046 & 22:17:21.47 & 0:14:54.6 & $>$27.0 & 26.43 & 1\secpoint8 & 1\secpoint8 & $<0.8$ & 3.100 \\
047 & 22:17:36.05 & 0:15:06.9 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.096 \\
048 & 22:17:27.37 & 0:16:51.5 & 26.73 & 26.00 & 2\secpoint2 & 1\secpoint7 & $0.5\pm0.2$ & 3.094 \\
049 & 22:17:39.29 & 0:16:10.5 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.094 \\
050 & 22:17:24.56 & 0:15:56.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.082 \\
051 & 22:17:33.72 & 0:15:04.9 & 26.26 & 27.21 & 0\secpoint3 & 0\secpoint7 & $2.4\pm1.3$ & 3.094 \\
052 & 22:17:36.84 & 0:13:17.2 & 26.63 & $>27.3$ & \ldots & \ldots & $>1.8$ & 3.102 \\
053 & 22:17:34.70 & 0:16:33.4 & 26.53 & 26.98 & 0\secpoint6 & 0\secpoint9 & $1.5\pm0.8$ & 3.090 \\
054 & 22:17:39.05 & 0:11:33.9 & 26.25 & $>27.3$ & \ldots & \ldots & $>2.6$ & 3.096 \\
055 & 22:17:35.80 & 0:11:50.0 & 26.67 & $>27.3$ & \ldots & \ldots & $>1.8$ & 3.072 \\
056 & 22:17:22.42 & 0:17:20.7 & 26.86 & $>27.3$ & \ldots & \ldots & $>1.5$ & 3.073 \\
057 & 22:17:25.40 & 0:10:58.3 & 26.84 & $>27.3$ & \ldots & \ldots & $>1.5$ & 3.070 \\
058 & 22:17:19.61 & 0:15:38.4 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
059 & 22:17:24.98 & 0:12:30.0 & 25.31 & $>27.3$ & \ldots & \ldots & $>6.2$ & 3.096 \\
060 & 22:17:28.19 & 0:11:17.1 & 26.61 & $>27.3$ & \ldots & \ldots & $>1.9$ & 3.065 \\
061 & 22:17:34.10 & 0:15:40.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.101 \\
062 & 22:17:22.87 & 0:14:41.7 & 26.53 & $>27.3$ & \ldots & \ldots & $>2.0$ & 3.057 \\
063 & 22:17:23.32 & 0:15:52.9 & 26.55 & $>27.3$ & \ldots & \ldots & $>2.0$ & 3.099 \\
064 & 22:17:35.42 & 0:12:14.6 & 26.05 & 26.74 & 0\secpoint1 & 1\secpoint0 & $1.9\pm0.9$ & 3.108 \\
065 & 22:17:28.15 & 0:14:36.4 & 26.91 & $>27.3$ & \ldots & \ldots & $>1.4$ & 3.102 \\
066 & 22:17:20.86 & 0:15:11.8 & 26.64 & $>27.3$ & \ldots & \ldots & $>1.8$ & 3.066 \\
067 & 22:17:36.26 & 0:13:11.7 & 26.40 & $>27.3$ & \ldots & \ldots & $>2.3$ & 3.106 \\
068 & 22:17:18.37 & 0:17:26.1 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.072 \\
069 & 22:17:18.96 & 0:11:12.0 & 24.62 & 27.22 & 0\secpoint2 & 0\secpoint9 & $10.9\pm5.1$ & 3.074 \\
070 & 22:17:39.28 & 0:14:00.2 & 25.98 & $>27.3$ & \ldots & \ldots & $>3.4$ & 3.090 \\
071 & 22:17:21.61 & 0:12:20.5 & 26.77 & $>27.3$ & \ldots & \ldots & $>1.6$ & 3.072 \\
072 & 22:17:31.24 & 0:17:32.1 & 27.00 & $>27.3$ & \ldots & \ldots & $>1.3$ & 3.084 \\
073 & 22:17:39.12 & 0:17:11.7 & 26.35 & $>27.3$ & \ldots & \ldots & $>2.4$ & 3.083 \\
074 & 22:17:36.47 & 0:12:54.8 & 26.16 & 25.52 & 0\secpoint1 & 0\secpoint7 & $0.6\pm0.2$ & 3.105 \\
075 & 22:17:22.97 & 0:11:25.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i} \\
076 & 22:17:20.67 & 0:15:13.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.066 \\
077 & 22:17:37.95 & 0:11:01.3 & 26.01 & 26.36 & 0\secpoint2 & 1\secpoint1 & \ldots & \ldots\tablenotemark{g} \\
078 & 22:17:37.68 & 0:16:48.3 & 25.95 & $>27.3$ & \ldots & \ldots & $>3.5$ & 3.090 \\
079 & 22:17:34.68 & 0:11:10.5 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.103 \\
080 & 22:17:35.95 & 0:13:43.3 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.104 \\
081 & 22:17:29.22 & 0:14:48.7 & $>$27.0 & 26.79 & 0\secpoint6\tablenotemark{j} & 0\secpoint7 & $<1.2$ & 3.104 \\
082 & 22:17:35.44 & 0:16:47.6 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.087 \\
083 & 22:17:28.46 & 0:12:08.9 & 26.46 & 26.84 & 0\secpoint4 & 0\secpoint6 & $1.4\pm0.7$ & 3.065 \\
084 & 22:17:19.90 & 0:15:14.9 & $>$27.0 & 26.50 & 0\secpoint1 & 0\secpoint8 & \ldots & \ldots\tablenotemark{i} \\
085 & 22:17:30.86 & 0:14:38.2 & 26.94 & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
086 & 22:17:28.42 & 0:13:42.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.100 \\
087 & 22:17:37.07 & 0:13:21.5 & $>$27.0 & 27.26 & 0\secpoint1\tablenotemark{j} & 1\secpoint6 & \ldots & \ldots\tablenotemark{g} \\
088 & 22:17:38.45 & 0:13:18.3 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
089 & 22:17:38.54 & 0:15:22.5 & 26.59 & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
090 & 22:17:18.25 & 0:14:06.4 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.095 \\
091 & 22:17:36.14 & 0:15:40.7 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.095 \\
092 & 22:17:23.97 & 0:15:27.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
093 & 22:17:27.48 & 0:13:57.5 & 26.35 & $>27.3$ & \ldots & \ldots & $>2.4$ & 3.106 \\
094 & 22:17:39.14 & 0:17:00.6 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
095 & 22:17:37.19 & 0:13:28.0 & 26.17 & $>27.3$ & \ldots & \ldots & $>2.8$ & 3.094 \\
096 & 22:17:38.93 & 0:11:37.4 & 26.64 & 26.45 & 0\secpoint6 & 0\secpoint6 & \ldots & \ldots\tablenotemark{g} \\
097 & 22:17:27.11 & 0:14:08.7 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.064 \\
098 & 22:17:24.01 & 0:13:19.5 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{g} \\
099 & 22:17:36.46 & 0:13:00.3 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.102 \\
100 & 22:17:30.61 & 0:18:11.6 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
101 & 22:17:25.33 & 0:17:22.5 & 26.89 & 26.58 & 0\secpoint2 & 1\secpoint4 & \ldots & \ldots\tablenotemark{g} \\
102 & 22:17:24.00 & 0:16:27.6 & 25.91 & 26.05 & 0\secpoint1 & 0\secpoint2 & \ldots & \ldots\tablenotemark{g} \\
103 & 22:17:19.40 & 0:15:26.1 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.099 \\
104 & 22:17:37.66 & 0:12:55.5 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.097 \\
105 & 22:17:35.46 & 0:12:23.9 & 26.81 & $>27.3$ & \ldots & \ldots & $>1.6$ & 3.104 \\
106 & 22:17:22.86 & 0:17:57.8 & 26.16 & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
107 & 22:17:20.96 & 0:14:46.7 & 26.57 & $>27.3$ & \ldots & \ldots & $>2.0$ & 3.075 \\
108 & 22:17:24.78 & 0:17:40.4 & 26.84 & $>27.3$ & \ldots & \ldots & $>1.5$ & 3.100 \\
109 & 22:17:23.98 & 0:17:57.8 & 26.77 & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{g}\\
110 & 22:17:19.50 & 0:15:57.6 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.074 \\
111 & 22:17:31.14 & 0:16:42.9 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.096 \\
112 & 22:17:32.72 & 0:15:54.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.096 \\
113 & 22:17:24.80 & 0:13:26.9 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.069 \\
114 & 22:17:34.50 & 0:14:20.0 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.103 \\
115 & 22:17:33.46 & 0:17:01.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.093 \\
116 & 22:17:28.00 & 0:12:14.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.096 \\
117 & 22:17:39.08 & 0:12:01.9 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.098 \\
118 & 22:17:35.28 & 0:10:59.9 & 26.20 & 26.11 & 0\secpoint4 & 1\secpoint4 & \ldots & \ldots\tablenotemark{g} \\
119 & 22:17:25.63 & 0:12:47.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.071 \\
120 & 22:17:26.76 & 0:10:59.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.079 \\
121 & 22:17:26.44 & 0:15:27.5 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.099 \\
122 & 22:17:38.19 & 0:14:03.7 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.106 \\
123 & 22:17:35.06 & 0:17:26.0 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
124 & 22:17:22.80 & 0:17:48.7 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{g} \\
125 & 22:17:38.02 & 0:14:03.6 & 26.79 & $>27.3$ & \ldots & \ldots & $>1.6$ & 3.101 \\
126 & 22:17:19.53 & 0:16:48.2 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & \ldots\tablenotemark{i}\\
127 & 22:17:36.91 & 0:11:27.1 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.107 \\
128 & 22:17:23.43 & 0:16:07.4 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.095 \\
129 & 22:17:22.28 & 0:10:57.9 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.111 \\
130 & 22:17:32.84 & 0:16:48.8 & $>27.0$ & $>27.3$ & \ldots & \ldots & \ldots & 3.092 \\
\enddata
\tablenotetext{a}{Spatial offset between the centroids of $R$ or Ly$\alpha$ and NB3640 emission.}
\tablenotetext{b}{Observed ratio and uncertainty in non-ionizing UV and LyC flux densities, inferred from the NB3640$-R$ color.  
This value has not been corrected for either contamination by foreground sources or IGM absorption.} 
\tablenotetext{c}{Spectroscopic redshift based on the observed wavelength of Ly$\alpha$ emission.}
\tablenotetext{d}{Objects that are also identified as LBGs. 001 is LBG D3; 002 is LBG C4;
004 is LBG MD23; 008 is LBG C28; 009 is LBG C9; 012 is LBG M28; 029 is LBG M13.}
\tablenotetext{e}{Objects with previously-known spectroscopic redshifts.}
\tablenotetext{f}{Spectrum contains evidence for the presence of a foreground galaxy.  Thus,
we do not consider the NB3640 detection to be LyC flux.}
\tablenotetext{g}{Objects with LRIS spectroscopic observations but without confirmed redshifts.}
\tablenotetext{h}{The redshift of this LAE is such that some non-ionizing UV flux will contribute
to the NB3640 detection, and therefore we exclude it from our LyC detection sample.}
\tablenotetext{i}{Objects without LRIS spectroscopic observations.}
\tablenotetext{j}{Offset determined from the centroid of the $BV$ detection.}

\end{deluxetable}


